FB$^+$-tree: A Memory-Optimized B$^+$-tree with Latch-Free Update

B$^+$-trees are prevalent in traditional database systems due to their versatility and balanced structure. While binary search is typically utilized for branch operations, it may lead to inefficient cache utilization in main-memory scenarios. In contrast, trie-based index structures drive branch operations through prefix matching. While these structures generally produce fewer cache misses and are thus increasingly popular, they may underperform in range scans because of frequent pointer chasing. This paper proposes a new high-performance B$^+$-tree variant called \textbf{Feature B$^+$-tree (FB$^+$-tree)}. Similar to employing bit or byte for branch operation in tries, FB$^+$-tree progressively considers several bytes following the common prefix on each level of its inner nodes\textemdash referred to as features, which allows FB$^+$-tree to benefit from prefix skewness. FB$^+$-tree blurs the lines between B$^+$-trees and tries, while still retaining balance. In the best case, FB$^+$-tree almost becomes a trie, whereas in the worst case, it continues to function as a B$^+$-tree. Meanwhile, a crafted synchronization protocol that combines the link technique and optimistic lock is designed to support efficient concurrent index access. Distinctively, FB$^+$-tree leverages subtle atomic operations seamlessly coordinated with optimistic lock to facilitate latch-free updates, which can be easily extended to other structures. Intensive experiments on multiple workload-dataset combinations demonstrate that FB$^+$-tree shows comparable lookup performance to state-of-the-art trie-based indexes and outperforms popular B$^+$-trees by 2.3x$\ \sim\ $3.7x under 96 threads. FB$^+$-tree also exhibits significant potential on other workloads, especially update workloads under contention and scan workloads.

==> section/response.tex <==
\section*{Response to Reviewer Comments}
Thank you to all the reviewers for your insightful advice, helpful comments, and encouragement regarding our paper. These valuable comments have provided important guidance and assistance in helping us improve the paper, and your affirmations would encourage our follow-up work. Our main revisions highlighted in blue in our revised manuscript are summarized as follows:

\vspace{0.5em}
\noindent
\textbf{\textit{Total Response.}}
\begin{enumerate}[left=0pt, label=\arabic*.]
    \item We have significantly polished the paper in Section \ref{section3} and \ref{section4}. In section \ref{feature-cmp}, we have heavily rewritten the expression of feature comparison technique. In addition, we have included Figure \ref{fig:comp} to illustrate the difference between traditional binary search and FB$^+$-tree's hybrid byte-wise processing branch algorithm and clarify when binary search on suffixes is required. \textbf{To our best knowledge, our FB$^+$-tree is the first to exploit byte-wise parallel processing in B$^+$-tree and to make SIMD vectorization enhanced B$^+$-tree extensively practical in main-memory database systems (novelty).} We must admit that FB$^+$-tree is not the first exploration of SIMD-enhanced index structures, while FB$^+$-tree exploits SIMD parallel processing quite differently from previous work and is more practical than previous work. Although previous work explores SIMD-enhanced B$^+$-tree, they still utilize binary search for branch operation. Instead, FB$^+$-tree uses byte-wise parallel processing for branch operation, which can heavily reduce dependences between instructions and thus can better exploit modern CPUs' parallelism potential. \par
    For example, FAST is a read-only binary tree that collapses multiple nodes into one large node to facilitate SIMD instructions. During each comparison in a large node, it compares several keys in an SIMD blocking and determines the offset to load data for the next SIMD comparison. It indicates a data dependence between two SIMD comparisons, which hinders instruction-level parallelism. FB$^+$-tree eliminates data dependence by instead sequentially performing byte-wise parallel processing. Meanwhile, prefixes can be skipped even for integer keys and much more keys can be parallelly compared in one SIMD instruction. We have illustrated the performance and hardware event statistics comparison in Figure \ref{fig:cache_miss}. In addition, collapsing multiple nodes into one large node makes it complicated and difficult to support efficient dynamic structure modification and indexing string keys (FAST utilizes compression techniques for string keys and it can not avoid false positives). But there is no such problem in FB$^+$-tree because in fact it is still a B$^+$-tree.  It leads to FAST and similar previous work (e.g. k-Ary, P-ary, etc.) being somewhat less practical than FB$^+$-tree in main-memory database systems. \label{resp:t1}
    
    \item \textbf{As for the latch-free update technique, FB$^+$-tree is the first index that combines CAS-based update with optimistic lock, as far as we know.} Compared with previous work, our latch-free update technique eliminates locking for update operations, while it does not incur additional overhead like merging in Bw-tree. To better clarify our synchronization protocol, we have heavily polished Section \ref{section4} by moving previous techniques into Section \ref{sync-primer} and illustrating their comparison with FB$^+$-tree's synchronization protocol in Table \ref{tab:sync}. In addition, we have simplified the description of other subsections of Section \ref{section4} to make it easier to understand.\label{resp:t2}

    \item For another important problem mentioned by the reviewers, the correlation among hardware event statistics, suffix comparisons, and performance of FB$^+$-tree with different feature sizes has been appropriately included in our revised manuscript, shown in Section \ref{sec:eva-opts} and Section \ref{sec:cmp-sota} (Figure \ref{fig:dif-fsize} and Figure \ref{fig:statistic}). Actually, we carefully selected the datasets, where rand-int represents some application scenarios with integer primary keys, such as auto-incrementing primary keys; 3-grams reflects some scenarios in large language models; ycsb represents random string keys; url represents very long keys tailored for trie's application scenarios; twitter is a real-world database dataset including primary keys traced from Twitter's production systems. Except for url dataset, FB$^+$-tree shows comparable point lookup performance to state-of-the-art index structures. For url dataset which has very long and various complicated prefix patterns and thus is more suitable to trie, we have to admit that FB$^+$-tree has lower performance because of more cache misses and suffixes comparisons, as shown in Figure \ref{fig:dif-fsize}, \ref{fig:statistic} and \ref{fig:indexes-ycsb} (but it still has higher performance than ART and Masstree). \label{resp:t3}

    \item We have included more experimental evaluations such as scan evaluation with actual record access (Figure \ref{fig:indexes-ycsb}) and update scalability under different skewness (Figure \ref{fig:skewed-update}), and have introduced more competitors such as FAST. The results illustrate that FB$^+$-tree still has better performance or scalability.\label{resp:t4}

    \item Paper reorganization: we reduced the length of the algorithm and related work, and included a lot of materials and experiments. (please see 1, 2, 3 and 4)
\end{enumerate}

\vspace{1em}
Next, we address the comments of each reviewer.\par
\textbf{R1:}\par
W1. \textit{The index was not build into a system.}\par
Response: While we did not build FB$^+$-tree into a system, we have included a scan evaluation with actual record access in our revised manuscript, which represents a significant portion of workloads in a real database system. This experiment actually goes beyond most of the same kind of previous work, which often overlooks the impact of record access on performance. In real systems, performance can be significantly influenced by various application contexts, including storage medium, network, and software stack. We are concerned that these factors may diminish the differences between these index structures in real systems. However, our experiments do take into account the performance of the indexing component across various workloads and aim to provide a fair comparison.

W2. \textit{No performance evaluation in a larger query context like TCP benchmarks.}\par
Response: While index structure is one of the most critical components in database systems, the TPC benchmark is domain-specific for different application scenarios. Therefore, it takes into account the combined impact of many components, such as concurrency control for transactions and record layout for analysis, both of which significantly affect the system's overall performance. But that is a very interesting question, and we will also try to apply FB$^+$-tree to a broader range of problems in main-memory database systems, and consider new research problems based on FB$^+$-tree as needed, such as index-based concurrency control and composed index.

D1. \textit{While I think it is acceptable for an index paper to run microbenchmarks on specific operations, seeing the performance benefits in a larger query context would be interesting.}\par
Response: In fact, we have included real database workloads, and while it follows the YCSB default Zipfian distribution, we suppose that everyone does, so it certainly represents the mainstream database application patterns. Specifically, we have included a set of scan experiments with actual record access in Figure \ref{fig:indexes-ycsb}.

D2. \textit{In some places, the text regarding the experimental results is somewhat misleading (in advantage of the proposed technique). For example, "Compared agains B+treeOLC ... FB+tree shows higher performance up to 2.3x to 3.7x." This is true, but does not mention that B+treeOLC is the worse preforming technique in this setting. If there is a reason to emphasize the performance advantage over B+treeOLC (e.g. as a B+tree representative) than it would be better to make it explicit.}\par
Response: Thank you for this helpful comment for helping us polish our paper. We have revised such expressions in our revised manuscript.


\vspace{2em}
\textbf{R2:}\par
W1. \textit{The presentation of the paper requires significant improvement. The description of previous work (e.g., optimistic lock coupling) is intermixed with the FB+-tree’s own concurrency protocol, making it challenging to differentiate the unique designs of the FB+-tree. Please refer to D2.}\par
Response: For your concern, we have heavily rewritten that section and responded in T\ref{resp:t2}. In addition, we have included another comparison Table \ref{tab:sync}, to emphasize the advantage of our latch-free update compared to previous synchronization protocols, shown in Section \ref{sync-primer}.

W2. \textit{The paper should provide detailed examples and figures to illustrate the feature comparison of FB+-tree. Please refer to D3.}\par
Response: This is a very important review for improving the paper. We have included a new Figure \ref{fig:comp}. We split Figure \ref{fig:comp} into three parts, as shown in the figure, our nodes are more compact and the overhead of hybrid branch algorithm is less than traditional binary search and totally byte-wise parallel processing. In addition, we have polished Section \ref{feature-cmp} to better clarify FB$^+$-tree's hybrid branch algorithm.

W3. \textit{The evaluation section should include a more in-depth analysis of the FB+-tree's performance advantages and more comprehensive experiments to better understand the effectiveness of proposed designs. Please refer to D4—D8.} \par
Response: This is a valuable comment for helping us polish the paper. We have responded in total response, please refer to T\ref{resp:t3}, T\ref{resp:t4} and R2:D4-D8.


D1: \textit{The design of the FB+-tree’s concurrency protocol is justified by highlighting the poor scalability of lock coupling in the B-link tree (Figure 2). However, since lock coupling is outdated for in-memory B+-trees, it should not serve as a primary motivation. Instead, the paper should demonstrate how traditional optimistic lock coupling is not scalable for update-intensive workloads and how FB+-tree addresses this issue through its lock-free update strategy.}\par
Response: Thanks for this insightful comment. We have updated Figure \ref{fig:scalability_latency} and have polished Section \ref{sec:intro-sync}. In detail, we have demonstrated that traditional lock coupling is poorly scalable for update-heavy workloads in contention.

D2. \textit{The technical sections are currently cumbersome to read and would benefit from a significant rewrite. Specifically, the paper should clearly separate the design of the FB+-tree from previous work and highlight its own contributions. For example, Sections 4.1 and 4.2 should focus more on the FB+-tree design rather than extensively illustrating previous methods such as the B-link tree and OLFIT. Previous techniques should be moved to a separate Background Section.}\par
Response: We have moved preliminaries to index synchronization into a separate subsection and polished other subsections in Section \ref{section4} to better clarify FB$^+$-tree's synchronization protocol. We have also responded in total response, please refer to T\ref{resp:t2}.

D3. \textit{The paper lacks clarity regarding when binary search on suffixes is required and when it is not after feature comparison. To address this, the paper should include more detailed figures and examples to better illustrate this aspect.}\par
Response: Thanks for this helpful comment. We have included a new Figure \ref{fig:comp} and polished Section \ref{feature-cmp} to better clarify FB$^+$-tree's hybrid branch algorithm. We have also responded in R2:W2.

D4. \textit{In Section 5.1, it is unclear whether the workload is skewed or uniform. The paper should also examine the update scalability of the FB+-tree and other indexes under varying levels of skewness.}\par
Response: We have emphasized the workload characteristics (Zipfian distribution with skew=0.99) in Section \ref{sec:exp-set}. We have also included a new experiment to evaluate the update scalability of different indexes under different skewness, as shown in Figure \ref{fig:skewed-update}. And the results illustrate that FB$^+$-tree has better performance and scalability in higher contention. Please see T\ref{resp:t2} and T\ref{resp:t3}.

D5. \textit{The analysis of performance advantages over other indexes is relatively superficial. A more detailed statistical analysis, including metrics such as cache misses and the number of suffix comparisons across different datasets, would provide a deeper understanding.}\par
Response: We have included such analysis in Section \ref{sec:cmp-sota}, as shown in Figure \ref{fig:dif-fsize} and Figure \ref{fig:statistic}. As we can see, indexes except for B$^+$-treeOLC have similar LLC misses, further confirming our experimental evaluation. We have also counted LLC-misses, suffix comparison and performance of FB$^+$-tree with different feature sizes in Figure \ref{fig:dif-fsize} and analyzed the reason why FB$^+$-tree's performance varies across different datasets in Section \ref{sec:eva-opts}. It shows that FB$^+$-tree with feature size 4 has better performance and space consumption, and we have detailed the reason in Section \ref{optimization}.  Please refer to T\ref{resp:t3}.

D6. \textit{The paper presents the range scan performance without accessing the actual key-value records, and the reason for this evaluation approach is not clearly justified. E.g., it is unclear whether this is real in practice. For completeness, the evaluation should include accessing and returning all key-value records.}\par
Response: Thanks for this helpful advice. We have included such experiments in Section \ref{sec:cmp-sota}. The results are shown in Figure \ref{fig:indexes-ycsb}. To our surprise, FB$^+$-tree has a certain superiority when performing range scan with actual record access. The reason is given in Section \ref{section2}. In addition, we add a scan\_simulation test program in our code to verify the superiority in range scan of FB$^+$-tree's lazy rearrangement in leaf nodes compared with wormhole's indirect ordered leaf node.


D7. \textit{The current evaluation only considers feature sizes of 2 and 4. A more comprehensive analysis, with a wider range of feature sizes and their corresponding performance impact (including hardware statistics and memory consumption), should be included.}\par
Response: We have included such evaluation in Figure \ref{fig:dif-fsize} and analyzed in Section \ref{sec:eva-opts}. Please also refer to R2:D5 and T\ref{resp:t3}.

D8. \textit{The results in Figure 8 show that FB+-tree performance varies across different datasets. It would be beneficial to analyze the factors within the datasets that influence the index’s performance.}\par
Response: We have illustrated the reason in Figure \ref{fig:dif-fsize} and analyzed in Section \ref{sec:eva-opts}. Please also refer to R2:D5 and T\ref{resp:t3}.


\vspace{2em}
\textbf{R3:}\par
W1. \textit{None of the optimizations used in the proposed method are particularly novel. Each technique has been applied in other index structures or other use cases in database area. So the overall technical contribution of the paper is somewhat limited, focusing more on combing existing techniques.}\par
Response: Please refer to T\ref{resp:t1} and T\ref{resp:t2}, the byte-wise parallel processing can efficiently exploit modern CPUs' instruction-level parallelism and data-level parallelism (processing more keys each comparison). In addition, this is the first implementation combining CAS-based update and optimistic lock, without additional overhead like merging in Bw-tree. The comparison with other synchronization protocols has been shown in Table \ref{tab:sync}.

W2. \textit{The choice of the STX B+-tree as a B-tree baseline is questionable, as it's unclear whether this implementation uses optimizations for modern CPUs, such as prefetching, SIMD vectorization, or advanced layouts. Given that there are several papers optimizing B+-tree for in-memory use on modern hardware, it's unclear if STX B+-tree represents the current state-of-the-art.}\par
Response: Thank you for this valuable comment. We have included such comparison in Figure \ref{fig:cache_miss}. Please refer to T\ref{resp:t1}. In detail, we have included FAST as a representative of SIMD-enhanced B-tree. The results demonstrate that FB$^+$-tree has less LLC misses and thus better performance than FAST.

W3. \textit{CAS is a widely used technique for implementing latch-free updates in index structures including B-tree. The paper doesn't clearly explain how the latch-free updates in FB+-tree differ from those in existing methods like BW-tree.}\par
Response: please refer to R3:W1 and total response T\ref{resp:t2}. In short, Bw-tree realizes lock-free operation through chaining delta records and a mapping table, which leads to heavy merging overhead and incurs additional overhead to lookup operations (FB$^+$-tree does not have such overhead). We have included Table \ref{tab:sync} to compare different synchronization protocols including Bw-tree.

D1. \textit{It seems that the latch-free update (Sec 4) is independent of the FB+-tree's index structure (Sec 3). Could these two components be evaluated separately? In Figure 8, does the performance include synchronization overhead (e.g, calling lock/unlock/CAS/etc), even though it's single-threaded execution?}\par
Response: So far, we consider latch-free update especially for FB$^+$-tree for the linked leaf node structure. It could be valuable to extend the idea to general use cases, for example, in ART, HOT, etc. However, another study is needed to solve the problem of its generality. In addition, that is true the performance of FB$^+$-tree and B$^+$-treeOLC include synchronization overhead in Figure \ref{fig:btree-ycsb} and the updated Figure \ref{fig:cache_miss}. But the performance of FAST and STXB$^+$-tree does not include such overhead. We suppose the performance of single-threaded FB$^+$-tree would be higher than its concurrent version evaluated in the paper. We will later implement a single-threaded version with more optimizations.

D2. \textit{Sec 5. What are the workload sizes? It's important for understanding FB+-tree's scalability and performance.}\par
Response: Suppose the reviewer is concerned about the key-value size, we have shown in Table \ref{tab:datasets}. Or the number of records, we have described in Section \ref{section5}, $10^8$ records, and all requests follow standard Zipfian distribution generated by YCSB with default parameters. Each workload has $10^8$ requests, and the run phase executes these requests for one minute for a more stable performance. For range scan operation, the scan length is also generated with default parameters, following uniform distribution and the average length is 50, as shown in Section \ref{section5}.

D3. \textit{Sec 5. Does STX B+-tree use the same fanout as FB+-tree?}\par
Response: We have to admit that their fanout factors are not exactly the same. The node size of STX B$^+$-tee is fixed by 256 bytes, and we also tried other configurations, but this default configuration delivers the best performance. FB$^+$-tree another intuition or advantage is optimizing tree height by using feature comparison technique and compact node. It is hard to make sure every competitor has the same fanout, but we try to make sure every competitor has the best performance.

M1. \textit{Figure 1: it would be clearer to show two separate bars for each event type.}\par
Response: Thanks for this helpful comment. We have updated Figure \ref{fig:cache_miss} and included a new competitor FAST in the micro-benchmark.

M2. \textit{Figure 1: why FB+-tree has fewer LLC misses compared to STX B+-tree?}\par
Response: Actually, FB$^+$-tree can reduce a lot of unnecessary memory access through prefix and feature comparison. We have detailed the reason in Section \ref{dissonance} and Section \ref{feature-cmp}. In addition, we have included a couple of Figures to illustrate hardware event statistics and suffix comparisons under different datasets, as shown in Figure \ref{fig:dif-fsize} and Figure \ref{fig:statistic}. Please refer to T\ref{resp:t3}.

M3. \textit{Sec 3.3: For AVX2, a fanout of 32 appears to be more optimal than 64, as 32 bytes align perfectly with the 256-bit register size.}\par
Response: While it's true that 32 bytes align perfectly with the 256-bit register size, our byte-wise parallel processing has very low computational overhead and the major overhead is memory access. So it has almost zero computational overhead to use a couple of AVX2 instructions to implement similar AVX512 instructions, especially modern CPUs have powerful instruction-level parallelism due to super-scalar, speculation, dynamic hardware scheduling, etc. Actually, FB$^+$-tree shows almost the same performance with different instruction sets (SSE2, AVX2, and AVX512). On this basis, a fanout of 32 leads to a deeper tree and therefore more cache misses and pointer chasing. As a result, we configure the fanout 64 even for AVX2 instruction set.
